DGAP: Efficient Dynamic Graph Analysis on Persistent Memory

Dynamic graphs, featuring continuously updated vertices and edges, have grown in importance for numerous real-world applications. To accommodate this, graph frameworks, particularly their internal data structures, must support both persistent graph updates and rapid graph analysis simultaneously, leading to complex designs to orchestrate `fast but volatile' and `persistent but slow' storage devices. Emerging persistent memory technologies, such as Optane DCPMM, offer a promising alternative to simplify the designs by providing data persistence, low latency, and high IOPS together. In light of this, we propose DGAP, a framework for efficient dynamic graph analysis on persistent memory. Unlike traditional dynamic graph frameworks, which combine multiple graph data structures (e.g., edge list or adjacency list) to achieve the required performance, DGAP utilizes a single mutable Compressed Sparse Row (CSR) graph structure with new designs for persistent memory to construct the framework. Specifically, DGAP introduces a \textit{per-section edge log} to reduce write amplification on persistent memory; a \textit{per-thread undo log} to enable high-performance, crash-consistent rebalancing operations; and a data placement schema to minimize in-place updates on persistent memory. Our extensive evaluation results demonstrate that DGAP can achieve up to $3.2\times$ better graph update performance and up to $3.77\times$ better graph analysis performance compared to state-of-the-art dynamic graph frameworks for persistent memory, such as XPGraph, LLAMA, and GraphOne.

==> 1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Graph-structured data are widely seen in real-world applications, such as social network, financial analysis, system security, and even storage systems~\cite{kwak2010twitter,zhou2016analyzing,albert1999diameter,jeong2000large,dai2014using}. Due to its importance, there have been numerous graph analysis frameworks designed in the literature. These efforts can be basically categorized into three classes: in-memory single-node frameworks, out-of-memory single-node frameworks, and distributed frameworks. 

As graph size grows quickly and graph-based applications become more demanding, existing graph analysis frameworks are facing significant challenges. For example, although the out-of-memory single-node or distributed frameworks can handle extremely large graphs, their performance is often an order of magnitude slower than that of the in-memory single-node frameworks due to the limited performance of external storage devices (e.g., SSD or HDD) and network communications. Such a performance degradation may be not acceptable to many applications, such as fraud detection or intrusion detection, which need the results ready in real-time or sub-seconds. 
%the state-of-the-art graph analysis framework LLAMA needs 7.9 seconds to perform BFS on Twitter graph purely in memory, but needs 233.8 seconds in the out-of-memory mode~\cite{macko2015llama}

%of vertices and several billion
On the other hand, although in-memory single-node frameworks can deliver needed performance with proper optimizations, they are significantly limited by the memory size of a single node and the volatile nature of in-memory graph store. In modern applications, graphs could easily reach a hundred billion edges~\cite{}. Even each edge only needs 16 bytes, storing the graphs will require more than 1.6TB memory space, making many in-memory graph frameworks impractical. Another major issue of in-memory frameworks is their graph data are volatile. The users have to deploy external services to guarantee the data persistence. This introduces significant overheads to synchronize the in-memory graph data structures with the external data sources: initially, the graph needs to be loaded into memory before analysis, which takes a long time to finish; later, any updates on the graph needs to be synchronized to the in-memory graph data structures, which is often done in batch to amortize the overheads of each synchronization. The batch updating basically prevents applications from running graph analysis on the latest graph, which again may be unacceptable to many applications.

In this study, we propose DGAP, a new single-node Dynamic Graph Analysis framework on Persistent memory, to address these issues. DGAP is designed to: 1) work with dynamic graphs up to trillions of edges on a single-node; 2) deliver graph analysis performance comparable to the in-memory graph analysis frameworks; 3) support continuously graph updates in a persistent and crash-consistent way. Deploying DGAP on a single node, users can grow their graphs to trillions of edges continously and run fast graph analysis upon the latest graph anytime, without worrying about data loss after a crash or reboot. 

To deliver these key functionalities, we root DGAP on persistent memory, particularly the Intel Optane DC Persistent Memory devices (PMEM for short)~\cite{inteloptane}. As a new storage device, PMEM provides both near-DRAM data access latency and data persistence capability~\cite{suzuki2015survey}. Plugged in the same slots, PMEM dimm provides much higher capacity (up to 512GB per dimm) than DRAM (64-128GB per dimm) via the same memory bus using CPU \verb|load| and \verb|store| instructions. Due to its high density, high performance, and persistence, PMEM is the key to realize the design goals of DGAP~\cite{qureshi2009enhancing,yang2013memristive,qureshi2009scalable}. 

%unfortunately  , due to the existence of CPU cache
Although PMEM is promising, simply converting existing in-memory or out-of-memory graph analysis frameworks into PMEM can not deliver the needed functionalities and performance. First, writing data into PMEM does not automatically guarantee data persistence. Hence simply operating the in-memory frameworks on PMEM regions does not provide the data persistence or crash consistency functionalities needed in DGAP. In fact, due to the existence of volatile CPU caches, PMEM write needs to be further flushed (e.g., \texttt{CLTFLUSHOPT}) and fenced (e.g., \texttt{sfence}) to guarantee persistence. In addition, a single PMEM write larger than 8 bytes may fail in the middle because the PMEM atomic write unit is 8 bytes. To enable crash consistency, proper extra handling is needed to recover from partial writes. 

Similarly, simply replacing the SSDs or HDDs used in existing out-of-memory frameworks with the faster PMEM devices does not lead to needed performance neither. There are multiple reasons: 1) the block-based I/O interfaces (POSIX or \texttt{MMAP}) introduce significant overheads, which diminish the benefit of using PMEM; 2) the graph data structures used in these out-of-memory frameworks are not optimized for PMEM device, which has asymmetric read/write performance, leading to low efficiency in data accesses.

DGAP is designed from scratch to work with PMEM natively. The core of DGAP is a new PMEM-friendly graph data structure designed based on Compressed Sparse Row (CSR) and Packed Memory Array (PMA) to enable fast data writes for graph updates and fast data reads for graph analytic tasks. DGAP introduces logging mechanism to further reduce the write amplifications and improve the write performance. It also includes detailed designs to enable data persistence and crash consistency. We prototype DGAP and compared its performance with state-of-the-art graph analysis frameworks running on PMEM across multiple graph analysis algorithms and real-world graphs. Our results show DGAP is able to deliver extremely fast performance on both graph updates and graph analysis. 

The remainder of this paper is organized as follows: In \S\ref{sec:background} we discuss several typical graph storage formats and their fits to temporal graphs. We introduce the concept of Packed Memory Array and the existing PMA-based CSR extension. In \S\ref{sec:design} and \S\ref{sec:operation} we present DGAP and its key components and operations in details. We present the extensive experimental results in \S\ref{sec:eval}. We compare with related work in \S\ref{sec:related}, conclude this paper and discuss the future work in \S\ref{sec:conclusion}.

%in both in-memory and out-of-memory modes

%The emerging storage technologies, e.g., Persistent Memory (PMEM), however, bring the potential features (e.g., low latency, high density, byte-addressable access) to overcome the challenges of the existing systems. These promising features bring the potentiality to solve the existing issues of both the in-memory and out-of-core graph processing systems. Unfortunately, this emerging storage device has limitations, too. For example, PMEM has read-write asymmetric performance (e.g., PMEM-write is ~3-4x slower than PMEM-read). Due to such limitations, a simple translation of the existing systems might not achieve the optimal performance.

% PMEM offers a higher density of memory at lower cost compared with DRAM, near-DRAM data access latency, and data persistence capability.

%In this research, our focus is to identify the limitations to port the existing graph processing systems in persistent memory and give a future research direction.

% developing a novel graph processing system that will perform optimally on this memory device.

%Graphs are widely seen in real-world applications, such as graph neural network, social network, financial analysis, system security, and even storage systems~\cite{kwak2010twitter,zhou2016analyzing,albert1999diameter,jeong2000large,dai2014using}. There are many graph analysis frameworks designed to support efficient processing on graphs. However, as applications evolve, existing graph analysis frameworks face various new challenges. 

%First, the size of the graphs increases quickly. It is not unusual for an application to handle graphs with multiple billion of edges, {\color{red} for example, xxx graph contains 1 billion of vertices and 16 billion of edges~\cite{}}. Even assuming each edge only takes 16 bytes to store its vertices and all properties, such a graph will take at least 256GB to store, making many in-memory graph analysis infeasible.

%Graph processing systems store these graphs and run different analytic algorithms to get insight from these data. Both of these tasks need to be done efficiently, as every data have a time to insight ranging from seconds to years. Meaning, after this time span, the data become less and less valuable. We need to store and analyze these data within this time window. Unfortunately, the design of the graph processing system is very challenging, because: (i) graphs are dynamic, meaning it needs to accept the incoming changes on the existing graph, (ii) graphs are huge, and (iii) graph analytic algorithms have irregular memory access pattern.

%Graphs are important in various applications. Nowadays, graphs become dynamic, need continuous updates and analyzed in real time. Also, graphs become much larger, harder to completely stay in DRAM

%This places significant challenges to the existing graph analysis systems. The in-memory graph analysis systems can not handle large graphs. It typically takes a long time for the in-memory graph analysis systems to load the data from external storage to DRAM each time. In addition, since the in-memory graph structures are often optimized for read, updating the DRAM graphs is typically complicated. Many of them can not take real-time updates into the system. They only accepted batch updates in a coarse granualrity.  On the other hand, the out-of-core graph analysis can handle large graphs. However, their performance is often much worse than their in-memory counterparts, providing limited capability to support real-time, high-performance graph analysis. 

%The recent emerging persistent memory devices open a new opportunity to support high-performance graph analysis on large-scale dynamic graphs. There are many different types of persistent memory technologies. The main one on the market is Intel Optane Persistent DRAM (PMEM). In this paper, we mainly focus on PMEM devices. First, PMEM provides much large storage space comparing with DRAM. The single PMEM dimm can provide upto 512GB 

%Graph analysis in a single node is done by either an in-memory or out-of-core manner. The in-memory graph analysis delivers the extreme performance 



%The existing graph processing systems can broadly categorize into three types: (i) DRAM based in-memory, (ii) out-of-core, and (iii) distributed. These systems have their own limitations. For example, DRAM capacity limits the in-memory systems, storage devices' bandwidth limits the out-of-core systems, and the expensive graph partitioning limits the distributed systems.

%As the graphs become larger and larger, in the near future, it would be in-practical to process graphs in the in-memory systems. Our major interest is the out-of-core systems, where graphs are stored in a secondary storage medium and move the pages in-memory while needed. Buffer pool and mmap are two options for such page maintenance working in user and kernel space respectively. As mentioned earlier, storage devices' bandwidth becomes the main bottleneck of such out-of-core systems.

%The emerging storage technologies, e.g., Persistent Memory (PMEM), however, bring the potential features (e.g., low latency, high density, byte-addressable access) to overcome the challenges of the existing systems. These promising features bring the potentiality to solve the existing issues of both the in-memory and out-of-core graph processing systems. Unfortunately, this emerging storage device has limitations, too. For example, PMEM has read-write asymmetric performance (e.g., PMEM-write is ~3-4x slower than PMEM-read). Due to such limitations, a simple translation of the existing systems might not achieve the optimal performance.

% PMEM offers a higher density of memory at lower cost compared with DRAM, near-DRAM data access latency, and data persistence capability.

%In this research, our focus is to identify the limitations to port the existing graph processing systems in persistent memory and give a future research direction.

% developing a novel graph processing system that will perform optimally on this memory device.

==> 2_background.tex <==
% \section{Graph Storage Formats and Dynamic Graphs}
\section{Background, Related Work, And Motivations}
\label{sec:background}

\subsection{Basic Graph Storage Formats}

\subsection{Out-of-memory Graph Systems}

\subsection{Motivation}
Many legacy graph storage systems (e.g., LLAMA and GraphChi) use mmap() system call to communicate with the persistent domain. As persistent memory also support mmap(), it enables the opportunity to use such legacy graph storage systems in the persistent memory without making any modifications. However, those legacy systems were targeted the traditional storage systems where mmap() achieves high performance, but that might not produce optimal performance in PMEM. For example, mmap() use msync() system call to synchronize changes to the storage media and msync() have known issue with handling smaller than page size flushes, unavailability of non-temporal (NT) stores, overhead of kernel system calls, and hugepages~\cite{aninvest2021iwata} which can be avoided in PMEM. For example, PMEM have other options (e.g., pmem\_persist() in pmdk library) to perform the similar operations (synchronize data with CPU instructions, such as CLWB or CLFLUSHOPT) that perform optimally in PMEM. So, although the existing legacy graph systems can operate on PMEM without any modification of the code, but it can not perform optimally on PMEM without modifications. Besides this, the graph analysis performance of these these graph storage systems heavily depends on the available memory in the system. For example, mmap loads the data on-demand to physical memory through page fault, keeps it in the page cache, and finally evicts those pages if memory fills up. So, more available memory means less eviction and page faults. However, PMEM is byte-addressable and loading data from PMEM bypasses the page cache, thus have no dependency on the available in the system.

Existing in-memory systems can also be used to PMEM, but it requires to modify the existing codes because:
To support the persistence guarantee in PMEM, it is necessary to apply PMEM-aware persistence guarantee supports. For example, pmdk have pmemobj\_persist(), pmemobj\_tx() functions to give persistence and transactional guarantees. Eventhough such a translation of in-memory system for persistent memory is not hard, but it might not produce optimal performance due to unique characteristics of PMEM. For example, PMEM have read-write asymmetry in performance, can not guarantee crash consistance in more than 8-bytes write. To achieve crash consistent support in more than 8-bytes write, PMEM require wither undo/redo logging based transactional support or careful system design for after crash recovery. As the logging can heavily degrade the the write performance, many systems prefer the later option (i.e., after crash recovery).


==> extra.tex <==
\begin{figure}[h!]
	\centering
	\includegraphics[width=0.5\textwidth]{figs/pcsr__write_shifts.pdf}
	\caption{\small Write amplification in PCSR.}
	\label{pcsr_write_amp}
\end{figure}

\begin{figure}[h!]
	\centering
	\includegraphics[width=0.5\textwidth]{figs/pcsr__write_shifts__comb.pdf}
	\caption{\small Write amplification in PCSR.}
	\label{pcsr_write_amp}
\end{figure}

\begin{figure}[h!]
	\centering
	\includegraphics[width=0.5\textwidth]{figs/vcsr__write_shifts.pdf}
	\caption{\small Write amplification in VCSR.}
	\label{pcsr_write_amp}
\end{figure}

\begin{figure}[h!]
	\centering
	\includegraphics[width=0.5\textwidth]{figs/vcsr__write_shifts__comb.pdf}
	\caption{\small Write amplification in VCSR.}
	\label{pcsr_write_amp}
\end{figure}



\begin{figure}[h!]
    \centering
    \begin{subfigure}[b]{1.0\linewidth}
    	\centering
    	\includegraphics[page=2,width=0.7\linewidth]{figs/vertex_update.pdf}
    	\label{fig:sub-first}
    \end{subfigure}
    % \vskip\baselineskip
    \begin{subfigure}[b]{1.0\linewidth}
    	\centering
    	\includegraphics[page=1,width=\linewidth]{figs/vertex_update.pdf}
    	\label{fig:sub-second}
    \end{subfigure}
    \caption{\small Time to update vertex array in dynamic CSR. \textit{The time to update 90\% of the dynamic edges in the Orkut graph. PMEM includes flush phase but does not have tx support. }}
    \label{eval:insert_vertex}
\end{figure}

\begin{figure*}[h!]
    \centering
    \begin{subfigure}[b]{1.0\linewidth}
    	\centering
    	\includegraphics[page=1,width=\linewidth]{exps/asplos23_2__multi_thread_analysis.pdf}
    	\label{fig:sub-first}
    \end{subfigure}
    % \vskip\baselineskip
    \begin{subfigure}[b]{1.0\linewidth}
    	\centering
    	\includegraphics[page=2,width=\linewidth]{exps/asplos23_2__multi_thread_analysis.pdf}
    	\label{fig:sub-second}
    \end{subfigure}
    \begin{subfigure}[b]{1.0\linewidth}
    	\centering
    	\includegraphics[page=3,width=\linewidth]{exps/asplos23_2__multi_thread_analysis.pdf}
    	\label{fig:sub-second}
    \end{subfigure}
    \begin{subfigure}[b]{1.0\linewidth}
    	\centering
    	\includegraphics[page=4,width=\linewidth]{exps/asplos23_2__multi_thread_analysis.pdf}
    	\label{fig:sub-second}
    \end{subfigure}
    \caption{\small Time to run graph algorithms on varying number of threads.}
    \label{eval:analytics_parallel}
\end{figure*}


\begin{table*}[h!]
    \resizebox{\textwidth}{!}{%
    % \small
	\centering
	\begin{tabular}{l cccccccccccccccccccc}
        \toprule & \multicolumn{10}{c}{PageRank} & \multicolumn{10}{c}{BFS} \\
        \cmidrule(lr){2-11}
        \cmidrule(lr){12-21}
        & \multicolumn{2}{c}{CSR} & \multicolumn{2}{c}{DGAP} & \multicolumn{2}{c}{BAL} & \multicolumn{2}{c}{LLAMA} & \multicolumn{2}{c}{GraphOne} & \multicolumn{2}{c}{CSR} & \multicolumn{2}{c}{DGAP} & \multicolumn{2}{c}{BAL} & \multicolumn{2}{c}{LLAMA} & \multicolumn{2}{c}{GraphOne}\\
        Graph     & $T_1$ & $T_{16}$ & $T_1$ & $T_{16}$ & $T_1$ & $T_{16}$ & $T_1$ & $T_{16}$ & $T_1$ & $T_{16}$ & $T_1$ & $T_{16}$ & $T_1$ & $T_{16}$ & $T_1$ & $T_{16}$ & $T_1$ & $T_{16}$ & $T_1$ & $T_{16}$\\
        \midrule
        %                   csr-1           csr-32          apma-1          apma-32         pcsr-1          pcsr-32         bal-1           bal-32          a/c-1               a/c-32              p/c-1               p/c-32
        Orkut          & 1(\num{24.17801})	& 1(\num{1.66891})	& \num{1.304939488}	& \num{1.322665692}	& \num{2.139864695}	& \num{2.096302377}	& \num{2.077962578}	& \num{5.700726822}	& \num{1.489278894}	& \num{1.574830278}	& 1(\num{0.33473})	& 1(\num{0.03006})	& \num{1.364353359}	& \num{1.283433134}	& \num{2.477339946}	& \num{2.20259481}	& \num{4.313924656}	& \num{11.01131071}	& \num{0.3565022555}	& \num{0.4134730539}\\
        
        Stackoverflow   & 1(\num{5.9909})	  & 1(\num{0.47123})	& \num{1.838096112}	& \num{2.021751586}	& \num{3.308022167}	& \num{3.189886043}	& \num{1.894540052}	& \num{3.236211616}	& \num{1.823966349}	& \num{1.741355601}	& 1(\num{0.38706})	& 1(\num{0.03287})	& \num{1.001188446}	& \num{1.01247338}	& \num{2.547434506}	& \num{2.804380894}	& \num{1.68449336}	& \num{13.26437481}	& \num{0.4866816514}	& \num{0.5055978096}\\

        Live-journal    & 1(\num{9.0714})	  & 1(\num{0.70642})	& \num{1.373577397}	& \num{1.326094958}	& \num{4.086972242}	& \num{3.841666431}	& \num{3.603082214}	& \num{7.25347527}	& \num{1.889994929}	& \num{1.751889811}	& 1(\num{0.34283})	& 1(\num{0.03262})	& \num{1.262404107}	& \num{1.144696505}	& \num{4.529533588}	& \num{3.950337216}	& \num{5.641279935}	& \num{15.45064378}	& \num{0.5762010326}	& \num{0.7853770693}\\

        Cit-Patents     & 1(\num{5.82708})	& 1(\num{0.4867})	  & \num{1.402165407}	& \num{1.297739881}	& \num{5.388343733}	& \num{4.635011301}	& \num{3.999258634}	& \num{5.806451613}	& \num{1.673489981}	& \num{1.444990754}	& 1(\num{0.4688}) 	& 1(\num{0.04374})	& \num{1.224765358}	& \num{1.0781893}	& \num{5.113929181}	& \num{4.26177412}	& \num{7.389078498}	& \num{15.43209877}	& \num{0.4148698805}	& \num{0.5726794696}\\
        \bottomrule
    \end{tabular}
    }

\resizebox{\textwidth}{!}{%
    % \small
	\centering
    \begin{tabular}{l cccccccccccccccccccc}
        & \multicolumn{10}{c}{BC} & \multicolumn{10}{c}{CC} \\
        \cmidrule(lr){2-11}
        \cmidrule(lr){12-21}
        & \multicolumn{2}{c}{CSR} & \multicolumn{2}{c}{DGAP} & \multicolumn{2}{c}{BAL} & \multicolumn{2}{c}{LLAMA} & \multicolumn{2}{c}{GraphOne} & \multicolumn{2}{c}{CSR} & \multicolumn{2}{c}{DGAP} & \multicolumn{2}{c}{BAL} & \multicolumn{2}{c}{LLAMA} & \multicolumn{2}{c}{GraphOne}\\
        Graph     & $T_1$ & $T_{16}$ & $T_1$ & $T_{16}$ & $T_1$ & $T_{16}$ & $T_1$ & $T_{16}$ & $T_1$ & $T_{16}$ & $T_1$ & $T_{16}$ & $T_1$ & $T_{16}$ & $T_1$ & $T_{16}$ & $T_1$ & $T_{16}$ & $T_1$ & $T_{16}$\\
        \midrule
        %                   csr-1           csr-32          apma-1          apma-32         pcsr-1          pcsr-32         bal-1           bal-32          a/c-1               a/c-32              p/c-1               p/c-32
        Orkut           & 1(\num{5.21541})	& 1(\num{0.42425})	& \num{1.034756615}	& \num{0.9836652917}	& \num{1.367714139}	& \num{1.254095463}	& \num{15.16026544}	& \num{13.46847378}	& \num{1.52932943}	& \num{1.370738951}	& 1(\num{2.60356})	& 1(\num{0.4192})	& \num{1.325830786}	& \num{1.734732824}	& \num{2.043882223}	& \num{1.977528626}	& \num{2.281491496}	& \num{2.063454198}	& \num{1.567592066}	& \num{1.791710401}\\
        
        Stackoverflow   & 1(\num{3.29676})	& 1(\num{0.24602})	& \num{0.8959523896}	& \num{1.026623852}	& \num{1.225742851}	& \num{1.233070482}	& \num{3.52618935}	& \num{3.381838875}	& \num{1.034175979}	& \num{0.9839565889}	& 1(\num{0.8761})	& 1(\num{0.44107})	& \num{1.302454058}	& \num{1.712494615}	& \num{2.804086292}	& \num{2.095993833}	& \num{1.490697409}	& \num{1.417008638}	& \num{1.636525511}	& \num{1.349588501}\\

        Live-journal    & 1(\num{4.37368})	& 1(\num{0.33103})	& \num{0.9674759013}	& \num{0.9613630185}	& \num{1.452975526}	& \num{1.416608767}	& \num{9.08136855}	& \num{8.334592031}	& \num{1.156225421}	& \num{1.082397366}	& 1(\num{0.9926})	& 1(\num{0.42197})	& \num{1.409419706}	& \num{1.893783918}	& \num{3.638373967}	& \num{2.580657393}	& \num{3.792061253}	& \num{2.77270896}	& \num{2.18112029}	& \num{1.777019693}\\
    
        Cit-Patents     & 1(\num{3.90332})	& 1(\num{0.29427})	& \num{0.8930397713}	& \num{0.8864648112}	& \num{1.350084031}	& \num{1.29303021}	& \num{6.333838886}	& \num{5.770211031}	& \num{0.9057264073}	& \num{0.8942739661}	& 1(\num{1.66957})	& 1(\num{0.48469})	& \num{1.402900148}	& \num{1.006086364}	& \num{4.632564073}	& \num{3.130743362}	& \num{3.172074247}	& \num{4.260455136}	& \num{1.967033428}	& \num{1.669671336}\\
        \bottomrule
    \end{tabular}
    }
    
    % % \resizebox{\textwidth}{!}{%
    % \begin{tabular}{l cccccccccccccccc}
    %     & \multicolumn{12}{c}{BFS} \\
    %     \cmidrule(lr){2-13}
    %     & \multicolumn{2}{c}{DGAP} & \multicolumn{2}{c}{BAL} & \multicolumn{2}{c}{LLAMA-5\%} & \multicolumn{2}{c}{LLAMA-1\%} & \multicolumn{2}{c}{GraphOne-1\%} & \multicolumn{2}{c}{GraphOne-2\%}\\
    %     Graph     & $T_1$ & $T_{32}$ & $T_1$ & $T_{32}$ & $T_1$ & $T_{32}$ & $T_1$ & $T_{32}$ & $T_1$ & $T_{32}$ & $T_1$ & $T_{32}$ \\
    %     \midrule
    %     %                   csr-1           csr-32          apma-1          apma-32         pcsr-1          pcsr-32         bal-1           bal-32          a/c-1               a/c-32              p/c-1               p/c-32
    %     Orkut          & \num{0.26652}	& \num{0.01745}	& \num{1.395842713}	& \num{1.170200573}	& \num{2.271274201}	& \num{1.963323782}	& \num{4.54776377}	& \num{7.711747851} &      \num{0.03386}	& \num{0.00211}	& \num{1.1497342}	& \num{1.255924171}\\
    %     Live-journal    & \num{0.26652}	& \num{0.01745}	& \num{1.395842713}	& \num{1.170200573}	& \num{2.271274201}	& \num{1.963323782}	& \num{4.54776377}	& \num{7.711747851} &      \num{0.03386}	& \num{0.00211}	& \num{1.1497342}	& \num{1.255924171}\\
    %     Cit-Patents     & \num{0.26652}	& \num{0.01745}	& \num{1.395842713}	& \num{1.170200573}	& \num{2.271274201}	& \num{1.963323782}	& \num{4.54776377}	& \num{7.711747851} &      \num{0.03386}	& \num{0.00211}	& \num{1.1497342}	& \num{1.255924171}\\
    %     Twitter         & \num{0.26652}	& \num{0.01745}	& \num{1.395842713}	& \num{1.170200573}	& \num{2.271274201}	& \num{1.963323782}	& \num{4.54776377}	& \num{7.711747851} &      \num{0.03386}	& \num{0.00211}	& \num{1.1497342}	& \num{1.255924171}\\
    %     Stackoverflow   & \num{0.26652}	& \num{0.01745}	& \num{1.395842713}	& \num{1.170200573}	& \num{2.271274201}	& \num{1.963323782}	& \num{4.54776377}	& \num{7.711747851} &      \num{0.03386}	& \num{0.00211}	& \num{1.1497342}	& \num{1.255924171}\\
    %     \bottomrule
    % \end{tabular}
    % % }
    
    % \begin{tabular}{l cccccccccccccccc}
    %     & \multicolumn{12}{c}{BC} \\
    %     \cmidrule(lr){2-13}
    %     & \multicolumn{2}{c}{DGAP} & \multicolumn{2}{c}{BAL} & \multicolumn{2}{c}{LLAMA-5\%} & \multicolumn{2}{c}{LLAMA-1\%} & \multicolumn{2}{c}{GraphOne-1\%} & \multicolumn{2}{c}{GraphOne-2\%}\\
    %     Graph     & $T_1$ & $T_{32}$ & $T_1$ & $T_{32}$ & $T_1$ & $T_{32}$ & $T_1$ & $T_{32}$ & $T_1$ & $T_{32}$ & $T_1$ & $T_{32}$ \\
    %     \midrule
    %     %                   csr-1           csr-32          apma-1          apma-32         pcsr-1          pcsr-32         bal-1           bal-32          a/c-1               a/c-32              p/c-1               p/c-32
    %     Orkut          & \num{0.26652}	& \num{0.01745}	& \num{1.395842713}	& \num{1.170200573}	& \num{2.271274201}	& \num{1.963323782}	& \num{4.54776377}	& \num{7.711747851} &      \num{0.03386}	& \num{0.00211}	& \num{1.1497342}	& \num{1.255924171}\\
    %     Live-journal    & \num{0.26652}	& \num{0.01745}	& \num{1.395842713}	& \num{1.170200573}	& \num{2.271274201}	& \num{1.963323782}	& \num{4.54776377}	& \num{7.711747851} &      \num{0.03386}	& \num{0.00211}	& \num{1.1497342}	& \num{1.255924171}\\
    %     Cit-Patents     & \num{0.26652}	& \num{0.01745}	& \num{1.395842713}	& \num{1.170200573}	& \num{2.271274201}	& \num{1.963323782}	& \num{4.54776377}	& \num{7.711747851} &      \num{0.03386}	& \num{0.00211}	& \num{1.1497342}	& \num{1.255924171}\\
    %     Twitter         & \num{0.26652}	& \num{0.01745}	& \num{1.395842713}	& \num{1.170200573}	& \num{2.271274201}	& \num{1.963323782}	& \num{4.54776377}	& \num{7.711747851} &      \num{0.03386}	& \num{0.00211}	& \num{1.1497342}	& \num{1.255924171}\\
    %     Stackoverflow   & \num{0.26652}	& \num{0.01745}	& \num{1.395842713}	& \num{1.170200573}	& \num{2.271274201}	& \num{1.963323782}	& \num{4.54776377}	& \num{7.711747851} &      \num{0.03386}	& \num{0.00211}	& \num{1.1497342}	& \num{1.255924171}\\
    %     \bottomrule
    % \end{tabular}
    
    % \begin{tabular}{l cccccccccccccccc}
    %     & \multicolumn{12}{c}{CC} \\
    %     \cmidrule(lr){2-13}
    %     & \multicolumn{2}{c}{DGAP} & \multicolumn{2}{c}{BAL} & \multicolumn{2}{c}{LLAMA-5\%} & \multicolumn{2}{c}{LLAMA-1\%} & \multicolumn{2}{c}{GraphOne-1\%} & \multicolumn{2}{c}{GraphOne-2\%}\\
    %     Graph     & $T_1$ & $T_{32}$ & $T_1$ & $T_{32}$ & $T_1$ & $T_{32}$ & $T_1$ & $T_{32}$ & $T_1$ & $T_{32}$ & $T_1$ & $T_{32}$ \\
    %     \midrule
    %     %                   csr-1           csr-32          apma-1          apma-32         pcsr-1          pcsr-32         bal-1           bal-32          a/c-1               a/c-32              p/c-1               p/c-32
    %     Orkut          & \num{0.26652}	& \num{0.01745}	& \num{1.395842713}	& \num{1.170200573}	& \num{2.271274201}	& \num{1.963323782}	& \num{4.54776377}	& \num{7.711747851} &      \num{0.03386}	& \num{0.00211}	& \num{1.1497342}	& \num{1.255924171}\\
    %     Live-journal    & \num{0.26652}	& \num{0.01745}	& \num{1.395842713}	& \num{1.170200573}	& \num{2.271274201}	& \num{1.963323782}	& \num{4.54776377}	& \num{7.711747851} &      \num{0.03386}	& \num{0.00211}	& \num{1.1497342}	& \num{1.255924171}\\
    %     Cit-Patents     & \num{0.26652}	& \num{0.01745}	& \num{1.395842713}	& \num{1.170200573}	& \num{2.271274201}	& \num{1.963323782}	& \num{4.54776377}	& \num{7.711747851} &      \num{0.03386}	& \num{0.00211}	& \num{1.1497342}	& \num{1.255924171}\\
    %     Twitter         & \num{0.26652}	& \num{0.01745}	& \num{1.395842713}	& \num{1.170200573}	& \num{2.271274201}	& \num{1.963323782}	& \num{4.54776377}	& \num{7.711747851} &      \num{0.03386}	& \num{0.00211}	& \num{1.1497342}	& \num{1.255924171}\\
    %     Stackoverflow   & \num{0.26652}	& \num{0.01745}	& \num{1.395842713}	& \num{1.170200573}	& \num{2.271274201}	& \num{1.963323782}	& \num{4.54776377}	& \num{7.711747851} &      \num{0.03386}	& \num{0.00211}	& \num{1.1497342}	& \num{1.255924171}\\
    %     \bottomrule
    % \end{tabular}
    
    \caption{\small The normalized running time of different algorithms (PageRank, BFS, BC, CC) on CSR, DGAP, BAL, LLAMA, and GraphOne. CSR is the baseline for all cases. We also add the actual runtime of CSR (in seconds). $T_1$ denotes the time of one thread and $T_{16}$ denotes the time of 16 threads.}
    \label{tab:normalized_algo}
    \vspace{-1em}
\end{table*}
